Graph-based Approach for Buffer-aware Timing Analysis of Heterogeneous Wormhole NoCs under Bursty Traffic

This paper addresses the problem of worst-case timing analysis of heterogeneous wormhole NoCs, i.e., routers with different buffer sizes and transmission speeds, when consecutive packet queuing (CPQ) occurs. The latter means that there are several consecutive packets of one flow queuing in the network. This scenario happens in the case of bursty traffic but also for non-schedulable traffic. Conducting such an analysis is known to be a challenging issue due to the sophisticated congestion patterns when enabling backpressure mechanisms. We tackle this problem through extending the applicability domain of our previous work for computing maximum delay bounds using Network Calculus, called Buffer-aware worst-case Timing Analysis (BATA). We propose a new Graph-based approach to improve the analysis of indirect blocking due to backpressure, while capturing the CPQ effect and keeping the information about dependencies between flows. Furthermore, the introduced approach improves the computation of indirect-blocking delay bounds in terms of complexity and ensures the safety of these bounds even for non-schedulable traffic. We provide further insights into the tightness and complexity issues of worst-case delay bounds yielded by the extended BATA with the Graph-based approach, denoted G-BATA. Our assessments show that the complexity has decreased by up to 100 times while offering an average tightness ratio of 71%, with reference to the basic BATA. Finally, we evaluate the yielded improvements with G-BATA for a realistic use case against a recent state-of-the-art approach. This evaluation shows the applicability of G-BATA under more general assumptions and the impact of such a feature on the tightness and computation time.

==> methodology.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Methodology of Buffer-aware approach
%  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In this section, we present the general ideas related to our buffer aware approach and develop the concepts that are common to both BATA and GRAPH models.
We first present the interest of buffer-aware approach on an example (\ref{subsec:illustrative_example}).
Then, we detail the formalism we will use (\ref{subsec:preliminaries}) and present the main steps of the method and the differences between the two approaches (\ref{subsec:main_steps}).
Finally, we recall the computation method of the direct blocking latency for a flow $f$, that will not be impacted by the extension of BATA approach, and illustrate it over an example.

\subsection{Illustrative Example}
\label{subsec:illustrative_example}

The key element to take into account the backpressure phenomenon induced by limited buffer size is based on how packets can spread in the network when stalled.  
We consider an illlustrative example to better understand the impact of the buffer size on the packet spreading, and consequently the indirect blocking set (Figure \ref{fig:intuitive_example_config}).  
We make the following assumptions: \begin{enumerate*}[label=(\roman*)]\item each buffer can store only one flit; \item all flows have 3-flit-long packets; \item all flows are mapped to the same VC; \item the \foi{} is flow 1.\end{enumerate*}

\begin{figure}[ht]
    \centering
    \resizebox{0.5\columnwidth}{!}{\input{WIP_intuitive_example.pdf_tex}}\resizebox{0.5\columnwidth}{!}{\input{WIP_intuitive_example_packet_detail.pdf_tex}}
    \caption{Example configuration (left) and packet stalling (right)}
    \label{fig:intuitive_example_config}
\end{figure}

We assume there is a packet A of flow 3 that has just been injected into the NoC and granted the use of the North output port of R6. 
Simultaneously, a packet B of flow 2 is reauesting the same output, but as A is already using it, B has to wait. 
B is stored in input buffers of R6, R5 and R4.
Finally, a packet C of flow 1 has reached R3 and now requests output port East of R3. However, the West input buffer of R4 is occupied by the tail flit of B.
Hence, C has to wait.
In that case, A indirectly blocks C, which means flow 3 can indirectly block flow 1 even though they do not share resources.


\begin{figure}[ht]
    \centering
    \resizebox{0.5\columnwidth}{!}{\input{WIP_problematic_example.pdf_tex}}\resizebox{0.5\columnwidth}{!}{\input{WIP_ib_example_single_packet_detail.pdf_tex}}
    \caption{Another configuration (left) where flow 1 cannot be blocked by flow 3 (right)}
    \label{fig:ib_example_single_packet}
\end{figure}
Now suppose flow 3 source is one hop further (Figure \ref{fig:ib_example_single_packet}). While the modification seems minor, it impacts the indirect blocking possibilities.
Consider that flow 3 has a packet A that has just been injected in the network and is using output port North of R7. As before, flow 2 has a packet B in the network that competes with A and has to wait. 
This time, however, the output requested by B is one hop further on flow 2 path. 
As a result, B is stored in input buffers of R7, R6 and R5.
Finally, flow 1 has injected a packet C into the NoC.
Since B is stalling one hop further than before on its path, C can request ouput port East of R3 and use input buffer West of R4, and reach its destination without contention.

An approach that does not consider buffer sizes would include flow 3 in the IB set of flow 1 regardless of the configuration. 
However, we just showed that it is not necessary.%\footnote{This relies on the assumption that there is no additional packet of 2 queueing right after B. We will develop this aspect later on.} 
This illustrates the impact of the buffer size on packet spreading.

Hence, the limited buffer size reduces the section of the path on which a blocked packet can in its turn block another one; thus the indirect blocking delay as well. 


\subsection{Preliminaries}
\label{subsec:preliminaries}
Consider $k$ and $l$ two flows that are directly interfering with one another, $\path_k, \path_l$ their paths, and let $\dv(\path_k, \path_l)$ be the last node they share :
\[ \dv(\path_k, \path_l) = \path_k[ \max \{i, \path_k[i] \in \path_l \}] \]
Suppose the path of $l$ continues after this node. Even if the head flit of $l$ is not stored in a router of $\path_{k} \cap \path_{l}$, the limited buffer size available in each router can lead to storing the tail flit of $l$ in a router of $\path_{k} \cap \path_{l}$ under contention. In that case, $l$ blocks $k$.

%However, we do have $\path_l[Last_l^k] = \path_k[Last_k^l] = \dv(k,l)$.
Therefore, we need to quantify the way a packet of flow $f$ spreads into the network when it is blocked and stored in buffers. 
Here, we assume node $r$ has a buffer size of $B_r$ to model heterogeneous architectures.
% Definition : spread index
\begin{Definition}
Consider a flow $f$ of maximum packet length  $L_{f}$ flits.
The spread index of $f$ at node $i$, denoted $N_{f}^i$, is defined as follows: 
%\[ N_f = \left\lceil \frac{L_{f}}{B} \right\rceil \]
\[ N_f^{i} = \min_{l \geq 0} \left\{ l, L_f \leq \sum\limits_{j = 0}^{l-1} B^{\path_f[i+j]} \right\} \]
where $B^r$ the buffer size at node $r$ in flits.
\label{def:spread_index}
\end{Definition}
%$N_{f}$ is the number of buffers needed to store one packet of flow $f$.
$N_f^i$ is the number of buffers needed to store one packet of flow $f$ from node $\path_f[i]$ onwards on the path of $f$.

Using this notion and the last intuitive example, we call the section of the path of flow $k$ from $\dv(\path_k, \path_l)$ through $N_k^{\dv(\path_k, \path_l)}$ nodes (at most) %after $\dv(\path_k, path_l)$ 
``subpath of $k$ relatively to $l$'':
\begin{Definition}
The subpath of a flow $k$ relatively to a flow $l$ is:
%\[ subpath(\path_k, \path_l) = \left[ \path_k[Last(\path_k,\path_l) + 1 ], \dots, \path_k[Last(\path_k,\path_l) + N_l] \right] \]
\begin{eqnarray*}
    subpath(\path_k,\path_l) &=& \Big[ \path_k[Last(\path_k,\path_l) + 1 ], \ldots, \\
                             & & \path_l[Last(\path_k,\path_l) + N_k^{Last(\path_k,\path_l) + 1} ] \Big] \\
\end{eqnarray*}
where $Last(\path_k,\path_l) = \max\{ n, \; \path_k[n] \in \path_l\}$ is the index of the last node shared by $k$ and $l$ along $\path_k$, i.e $\path_k[Last(k,l)] = \dv(k,l)$. 
\label{def:subpath1}
\end{Definition}
We can extend this notion and define, in a similar fashion, the subpath of any flow $k$ relatively to a subpath $\subpath_l \subset \path_l$ of any flow $l$ (with $l\neq k$ or $l=k$).
The previous notation still holds:
\begin{Definition}
The subpath of a flow $k$ relatively to any subpath $\subpath_l$ of any flow $l$ is:
\begin{eqnarray*}
    subpath(\path_k, \subpath_l) &=& \Big[ \path_k[Last(\path_k, \subpath_l) + 1 ], \ldots, \\
           & & \path_k[Last(\path_k, \subpath_l) + N_k^{Last(\path_k,\subpath_l) + 1}] \Big] 
\end{eqnarray*}
where $Last(\path_k,\subpath_l) = \max\{ n, \; \path_k[n] \in \subpath_l\}$ is the index along $\path_k$ of the last node shared by $k$ %on $\path_k$ 
and $l$ within $\subpath_l$.
By abuse of notation, we may denote $subpath(k,l)$ to refer to $subpath(\path_k,\path_l)$, and similarly $subpath(k, \subpath_l)$ to refer to $subpath(\path_k,\subpath_l)$.
\end{Definition}

It is worth noticing that if $\path_l$ ends before reaching the $N_l^{Last(\path_k,\path_l) + 1}$-th node after $\dv(\path_k,\path_l)$, then we ignore the out-of-range indexes. The notion of subpath is illustrated in Figure \ref{fig:subpath} for the \foi{} $k$ and a spread index for the interfering flow $l$ right after node $\dv(\path_k, \path_l)$ equal to 3, \ie{}, $N_l^{Last(\path_k, \path_l) + 1} =3$.

% TODO: replace with WIP example ?
\begin{figure}[ht]
\centering
\resizebox{\columnwidth}{!}{\input{NC_model_subpath.pdf_tex}}
\caption{Subpath illustration for the \foi{} $k$}
\label{fig:subpath}
\end{figure}

We will also need the following definitions.
\begin{Definition}
Let $f$ be the \foi{}. The set of flows that share resources with $f$ on their paths is called the Direct Blocking set of $f$ and denoted $DB_f$. Moreover, the subset of flows in $DB_f$ sharing resources with $f$ along $path$ is denoted $DB_f^{|path}$.  
\end{Definition}
\begin{Definition}
Let $f$ be the \foi{}. 
$hp(f)$ is the set of flows mapped to a VC of strict higher priority than $f$.
$sp(f)$ is the set of flows mapped to the same VC as $f$, $f$ excluded.
$lp(f)$ is the set of flows mapped to a VC of strict lower priority than $f$.
Morevoer, we define $slp(f) = sp(f) \cup lp(f)$ (resp. $shp(f) = sp(f) \cup hp(f)$), that is all flows with a priority lower or equal (resp. higher or equal) than $f$, $f$ excluded.
\end{Definition}

\begin{Definition}\label{def:ibset}
The indirect blocking set of a flow $f$ is the set of flows that do not physically share any resource with the \foi{}, but cause a delay to the \foi{} because they impact (directly or indirectly) at least one flow of $DB_f$. 
It is denoted $IB_f$ and contains pairs of the form \{flow id, subpath\} to specify, for each flow, where a packet of that flow can cause blocking that may propagate to the \foi{} through backpressure.
\end{Definition}

It is worth noticing that Definition \ref{def:ibset} is slightly different from the one used in the Scheduling Theory approaches \cite{burns_priority_share} \cite{liu_tighter_time_analysis}, where there is a distinction between the indirect blocking, due to same-priority flows, and indirect interference, due to higher priority flows. In our approach, we only consider flows belonging to the same VC as the \foi{} to compute the indirect blocking set, since the impact of higher priority flows is already integrated in our model as follows:
\begin{itemize}
    \item if a higher priority flow blocking our \foi{} gets blocked, the \foi{} can bypass it. In this case, we take into account the extra processing delay needed to allocate the shared resource to the \foi{}. On the other hand, the buffer backpressure will only propagate among flows from the same class, as illustrated in Figure \ref{fig:bypass};
    \item the influence of higher priority flows on the same priority flows than the \foi{}, which are inducing the indirect blocking, is modeled through the granted end-to-end service curve of each one of these flows at the rate and latency levels, as explained in Section \ref{subsec:direct_blocking_latency}
     %indirectly-blocking same priority flows is taken into account through the use of residual service curves. 
\end{itemize}


\subsection{Main Steps of Timing Analysis}
\label{subsec:main_steps}

To get a bound on the end-to-end latency for a flow $f$, we first need to compute its end-to-end service curve.
%As explained in \cite{giroudot_buffer_aware}, 
The end-to-end service curve of $f$ is denoted:
\[ \beta_{f}(t) = R_f \left( t - T_f \right)^+ \]
% And we have :
% \begin{equation}
% \label{Tf}
% T_f = T_{DB} + T_{IB} + T_{\path_f}
% \end{equation}
where $T_f$ is the sum of:
\begin{itemize}
    \item $T_{\path_f}$, the ``base latency'', that any flit of $f$ experiences along its path due only to the technological latencies of the crossed routers; %For convenience, we include it in $T_{DB}$ from here on;
    \item $T_{DB}$, the maximum direct blocking latency, due flows in $DB_f$;% to interference by flows sharing resources with the flow of interest;
    \item $T_{IB}$, the maximum indirect blocking latency, due to flows in $IB_f$. %that can indirectly block $f$ through the buffer backpressure phenomenon.%, and these flows are denoted \textit{indirect blocking} set $IB_f$.
\end{itemize}

% In the case of a Fixed-Priority Arbitration between VCs, we denote $T_{DB}$ as :
% \[ T_{DB} = T_{hp} + T_{sp} + T_{lp} \]
% \begin{itemize}
%     \item $T_{hp}$ is part of the maximum direct blocking latency, due to flows of higher priority sharing resources with $f$, which are part of the \textit{direct blocking} set $DB_f$;
%     \item $T_{sp}$ is part of the maximum direct blocking latency, due to same priority flows sharing resources with $f$, and also part of $DB_f$ set;
%     \item $T_{lp}$ is part of the maximum direct blocking latency, due to flows of lower priority sharing resources with $f$, and also part of $DB_f$ set;
% \end{itemize}

For now, we remain oblivious of how to use the indirect blocking set to derive the corresponding latency. This aspect will be covered in the next sections.

To compute the bound on the end-to-end latency for the \foi{}, we proceed according to Algorithm \ref{alg:end_to_end_service_computation} :
\begin{enumerate}
    \item We compute $T_{\path_f}$ (Line \ref{lin:T_P_f}), then $T_{DB}$ (Lines \ref{lin:T_DB_start} to \ref{lin:T_DB_end});
    \item We run our indirect blocking analysis and extract the IB set (Line \ref{lin:IB_f});
    \item We compute $T_{IB}$ (Lines \ref{lin:T_IB_start} to \ref{lin:T_IB_end}). 
    \item From there on, we know the end-to-end service curve for $f$ (Line \ref{lin:beta_f}). Thus all that is left is to compute the end-to-end delay bound using Theorem \ref{TH1} :
\begin{equation}
\label{eed}
D_f^{\path_f} = \frac{\sigma^{\path_f[0]}}{R_f} + T_{hp} + T_{sp} + T_{lp} + T_{IB} + T_{\path_f} 
\end{equation}
where $\sigma^{\path_f[0]}$ is the burst of the initial arrival curve of $f$ (the arrival curve of $f$ at node $\path_f[0]$, \ie{} the first node of its path).
\end{enumerate}

\begin{algorithm}
\caption{Computing the end-to-end service curve for a flow $f$}
\label{alg:end_to_end_service_computation}
endToEndServiceCurve($f, \path_f$)
\begin{algorithmic}[1]
    \STATE Compute $R_f$
    \STATE Compute $T_{\path_f}$ \label{lin:T_P_f}\\

    \COMMENT{Compute $T_{DB}$:}
    \STATE $T_{DB} \leftarrow 0$ 
    \FOR{$k \in DB_f$}\label{lin:T_DB_start}
        \STATE $r_0 \leftarrow \conv(k,f)$ \COMMENT{Get convergence point of $f$ and $k$}
        \STATE $\beta_k \leftarrow $ endToEndServiceCurve($k, [\path_k[0], \cdots, r_0]$)\label{lin:recursive_db}
        \STATE $\alpha_k^0 \leftarrow $ initial arrival curve of $k$
        \STATE $\alpha_k \leftarrow \alpha_k^0 \oslash \beta_k$
        \STATE $T_{DB} \leftarrow $ directBlocking($\alpha_k^{r_0}$)
    \ENDFOR\label{lin:T_DB_end}

    \COMMENT{Compute $T_{IB}$:}
    \STATE Compute $IB_f$ according to approach\label{lin:IB_f}
    \STATE $T_{IB} \leftarrow 0$\label{lin:T_IB_start}
    \FOR{$\{k,S\} \in IB_f$}
        \STATE $\widetilde{\beta}_k \leftarrow$ VC-service curve of $k$ on $S$\\
        %\COMMENT{Propagate arrival curve at the beginning of $S$ :}
        %\STATE $r_0 \leftarrow S[0]$
        %\STATE $\beta_k \leftarrow $ endToEndServiceCurve($k, [\path_k[0], \cdots, r_0]$)
        %\STATE $\alpha_k^0 \leftarrow $ initial arrival curve of $k$
        %\STATE $\alpha_k \leftarrow \alpha_k^0 \oslash \beta_k$\\
        \STATE $\alpha_k \leftarrow$ arrival curve of $k$ according to approach \label{lin:subpath_arrival_curve}\\
        \COMMENT{Now add the latency over the subpath to $T_{IB}$ :}
        \STATE $T_{IB} \leftarrow T_{IB} + h(\alpha_k, \widetilde{\beta}_k) $
    \ENDFOR\label{lin:T_IB_end}

    \RETURN $\beta = R_f (t - (T_{\path_f} + T_{DB} + T_{IB}))^+$\label{lin:beta_f}
\end{algorithmic}
\end{algorithm}

We summarize the differences between the two approaches we will detail in the next sections. As shown on Figure \ref{fig:comparative_approach}, the steps are similar but two of them are done differently according to the approach.
\begin{figure}[ht]
\centering
\resizebox{\columnwidth}{!}{\input{NC_model_approach_comparative_synthesis.pdf_tex}}
\caption{Computing end-to-end service curve latency : comparative of BATA and GRAPH approach.}
\label{fig:comparative_approach}
\end{figure}

\subsection{Direct Blocking Latency Computation}
\label{subsec:direct_blocking_latency}

The direct blocking latency takes into account the impact of flows sharing resources with the \foi{}. %As mentioned earlier, we also include the technological latency in $T_{DB}$.
We used PMOO \cite{schmitt_pmoo} to account for flow serialization phenomena when computing the maximum direct blocking latency.
As introduced in \cite{giroudot_buffer_aware}, it is defined in the following Theorem.
%=====================================================================================================================
\begin{Theorem}
\label{Th:directblocking}(Maximum Direct Blocking Latency)\\
The maximum direct blocking latency for a \foi{} $f$ along its path $\path_f$,  in a NoC under flit-level preemptive FP multiplexing with strict service curve nodes of the rate-latency type $\beta_{R,T}$ and leaky bucket constrained arrival curves $\alpha_{\sigma, \rho}$ is equal to:
 \[T_{\path_f} +T_{hp} + T_{sp} + T_{lp}\] 

with:
%========================================================================================================================================================
\begin{subequations}
\label{directBlocking}
\begin{align}
%&  T_{\path_f} = \sum\limits_{r \in \path_f} T^r \\
&  T_{hp} =  \sum\limits_{i \in DB_f \cap hp(f)} \frac{\sigma_i^{\conv(i,f)} + \rho_i \cdot \sum\limits_{r \in \path_f \cap \path_i} \left( T^r + \frac{ L_{slp(f)}^{r} }{R^{r}} \right)}{R_f}  \\
&  T_{sp} =  \sum\limits_{i \in DB_f \cap sp(f)} \frac{\sigma_i^{\conv(i,f)} + \rho_i \cdot \sum\limits_{r \in \path_f \cap \path_i} \left( T^r + \frac{ L_{slp(f)}^{r} }{R^{r}} \right)}{R_f}  \\
& T_{lp} = \sum\limits_{r \in \path_f} \frac{L_{slp(f)}^{r} }{R^{r}} 
\end{align}
\end{subequations}

where:
\begin{subequations}
\label{directBlockingvariables}
\begin{align}
&  L_{slp(f)}^{r} = \max\left( \max\limits_{j \in sp(f)} \left( L_{j} \cdot \mathbf{1}_{\{sp(f) \supset r\}} \right) \, , S_{flit} \cdot \mathbf{1}_{\{lp(f) \supset r \}} \right) \nonumber \\
&  R_f =  \min\limits_{r \in \path_f} \left\{ R^r - \sum\limits_{j \ni r, j \in shp(f)} \rho_j \right\} \nonumber
\end{align}
\end{subequations}
\end{Theorem}
The proof can be found in \cite{giroudot_buffer_aware}. 

\begin{application}
    We now detail the computations on the example of Figure \ref{fig:<++>}, for the \foi{} 1. 
    We assume all routers have a service curve $\beta = R (t - T)^+$ and flow $i$ has a packet length $L_i = L$ and the initial arrival curve $\alpha_i = \sigma + \rho t$.
    All flows are mapped to the same VC, thus $T_{hp} = T_{lp} = 0$. 
    We then have :
    \begin{eqnarray*}
	    T_{\path_1} &=& 4 T\\
	    T_{sp}      &=& \frac{\sigma_2^{R3} + \rho (\cdot T + \frac{L_i}{R})}{R - \rho} \\
	    &=& \frac{\sigma + \rho \cdot (T + \frac{L}{R})}{R - \rho} \\
    \end{eqnarray*}

    Hence :
    \begin{eqnarray*}
    T_{DB} &=& 4 T + \frac{\sigma}{R - \rho} + \rho\frac{ T + \frac{L}{R} }{R - \rho}\\
           &=& 7,368421053 \textrm{ cycles}
    \end{eqnarray*}
    with $R = 1$ flit/cycle, $T = 1$ cycle, $\rho = 0.05$ flits/cycle, $\sigma = 3$ flits and $L = 3$ flits.
\end{application}

It is important to notice that when we compute the direct blocking latency $T_{DB}$ of the \foi{}, we need to know the burst of interfering flows at their convergence point with the \foi{}.
Thus we need to compute, for each interfering flow, its service curve from its source to the aforementioned convergence point.

The end-to-end service curve computation is thus a recursive process (cf. Algorithm \ref{alg:end_to_end_service_computation}).
The recursion terminates because each call to endToEndServiceCurve() is done upstream the current convergence point.


==> network_calculus.tex <==
%%%%%%%%%%%%%%%%
% 
% NC Background
% 
%%%%%%%%%%%%%%%%


Network Calculus describes data flows by means of cumulative functions, defined as the number of transmitted bits during the time interval $[0, t]$.
%These functions are non negative and wide sense increasing:
%\begin{displaymath}
%\mathcal{F}=\{ f: \mathbb{R}^+ \rightarrow \mathbb{R}^+ \mid f(0)=0, \forall t \geq s: f(t) \geq f(s) \}
%\end{displaymath}
Consider a system $S$ receiving input data flow with a Cumulative Arrival Function (CAF), $A(t)$, and putting out the same data flow with a Cumulative Departure Function (CDF), $D(t)$. %Furthermore, $S$ fulfills the causality condition, \ie{}, $\forall t \in \mathbb{R}^+, A(t) \geq D(t)$. Then, at the instant $t$, the delay and backlog are simply the vertical and horizontal distances between $A(t)$ and $D(t)$, respectively.
To compute upper bounds on the worst-case delay and backlog, we need to introduce the maximum arrival curve, which provides an upper bound on the number of events, e.g., bits or packets, observed during any interval of time.
%Consequently, this curve covers all possible scenarios of traffic arrivals, observed at any instant, \ie{}, if $\alpha$ is a maximum arrival curve, then for any interval duration $\Delta$, there will be at most $\alpha(\Delta)$ events.
%This concept allows modeling a large panel of event arrival patterns, such as periodic, sporadic, with or without jitter or burst.
\begin{Definition}
\label{AC-def}
(Arrival Curve)\cite{le_boudec_thiran_nc_book} A function $\alpha$ is an arrival curve for a data flow with the CAF $A$, iff:
%\begin{equation}
\[ \forall t,s \geq 0, s\leq t, A(t) - A(s) \leq \alpha(t-s) \]
%\end{equation}
\end{Definition}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure}[h!]
% \centering
% \includegraphics[scale=0.4]{images/arrivalCurve3.jpg}
% \caption{\it Arrival curve}
% \label{ArrivalCurve}
% \end{figure}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%The arrival pattern necessary to define the maximum arrival curve can be obtained from traffic traces if any, or application's specification. The latter is more common for real-time communication networks.
A widely used curve is the leaky bucket curve, which guarantees a maximum burst $\sigma$ and a maximum rate $\rho$, \ie{}, the traffic flow is $(\sigma,\rho)$-constrained. In this case, the arrival curve is defined as $\gamma_{\sigma, \rho} (t)= \sigma+ \rho\cdot t$ for $t >0$.
%\subsection{Service Curves}
%\label{NMH}
%To conduct worst-case performance analysis, we need to put constraints on the input traffic through the maximum arrival curve notion. In return,
Furthermore, we need to guarantee a minimum offered service within crossed nodes through the concept of minimum service curve.
\begin{Definition}
\label{SC-def}
(Simple Minimum Service Curve)\cite{le_boudec_thiran_nc_book} The function $\beta$ is the simple service curve for a data flow with the CAF $A$ and the CDF $D$, iff:
%\begin{equation}
\[ \forall t \geq 0,D(t) \geq \inf_{s \leq t} (A(s)+ \beta(t-s)) \]
%\end{equation}
\end{Definition}
A very useful and common model of service curve is the rate-latency curve $\beta_{R,T}$, with $R$ the minimum guaranteed rate and $T$ the maximum latency before starting the service. This rate-latency function is defined as $\beta_{R,T}(t)= [R\cdot(t-T)]^+$, where $\left[x\right]^+$ is the maximum between $x$ and $0$.
%This service curve is easy to define in the case of \textit{one input/output node} serving one or many traffic flows coming from the same source and going to the same destination.
%Moreover, to model a node implementing aggregate scheduling, \ie{}, multiplexes the crossing flows at the input and demultiplexes them at the output, we need to define the \textit{left-over service curve} guaranteed to each flow within the crossed node, considering the impact of contention with other traffic flows. The computation of such a left-over service curve depends on the implemented scheduling policy, and its derivation needs strict service curve property in the general case.
%%A minimum strict service curve is defined as:
%\begin{Definition}
%\label{def:strict-service-curve}
%(Strict service curve)\cite{le_boudec_thiran_nc_book} The function $\beta $ is a strict service curve for a data flow with the CDF $D(t)$, if for any backlogged period \footnote{A backlogged period $]s,t]$ is an interval of time during which the backlog is non null, \ie{}, $A(s)=D(s)$ and $\forall u \in ]s,t]$, $A(u)-D(u) > 0$} $]s,t]$, $D(t) - D(s) \geq \beta(t-s)$.
%\end{Definition}
%The main results concerning the left-over service curves computation are as follows:
%\begin{Theorem} (Left-over service curve - Arbitrary Multiplex)\cite{bouillard2009service}
%\label{thm:residual-service-curve}
% let $f_1$ and $f_2$ be two flows crossing a server that offers a strict service curve $\beta$ such that $f_1$ is $\alpha_1$-constrained, then the left-over service curve offered to $f_2$ is:
%\begin{displaymath}
%\beta_2= (\beta - \alpha_1)_{\uparrow}
%\end{displaymath}
%where  $f_{\uparrow}(t) = \max\{0,\sup_{0 \leq s \leq t} f(s)\}$
%\end{Theorem}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{Corollary}(Left-over service curve - FP Multiplex)\cite{bouillard2011packetization}
%\label{cor:residual-sc}
%Consider a system with the strict service $\beta$ and $m$ flows crossing it, $f_1$,$f_2$,..,$f_m$. The maximum packet length of $f_i$ is $l_{i,max}$ and $f_i$ is $\alpha_i$-constrained. The flows are scheduled by the non-preemptive fixed priority (NP-FP) policy, where $f_i \succ f_j \Leftrightarrow i < j$. For each $i \in \{2,..,m \}$, the strict service curve of $f_i$ is given by:
%%\begin{equation}
%\[ (\beta - \sum_{j <i} \alpha_j - \max_{k \geq i} l_{k,max})_{\uparrow} \]
%%\end{equation}
%\end{Corollary}
%
%\subsection{Performance Bounds}
%\label{PAN}

Knowing the arrival and service curves, one can compute the upper bounds on performance metrics for a data flow, according to the following theorem.
\begin{Theorem} (Performance Bounds)
\label{TH1}
Consider a flow constrained by an arrival curve $\alpha$ crossing a system $\mathcal{S}$ that offers a service curve $\beta$, then:\\
 Delay \footnote{$h(f,g)$: the maximum horizontal distance between $f$ and $g$}: $ \forall~t:~d(t)\leq h(\alpha,\beta)$ \\
Backlog \footnote{$v(f,g)$: the maximum vertical distance between $f$ and $g$}: $ \forall~t:~q(t)\leq v(\alpha,\beta)$ \\
Output arrival curve \footnote{$f \oslash g(t) = \sup_{\forall u \geq 0} \{ f(t+u) - g(u)\}$}: $\alpha^*(t) =\alpha \oslash\beta (t)$
\end{Theorem}

In the case of a leaky bucket arrival curve and a rate-latency service curve, the calculus of these bounds is greatly simplified. The delay and backlog are bounded by $\frac{\sigma}{R} + T$ and $ \sigma + \rho \cdot T$, respectively; and the output arrival curve is $\sigma+ \rho \cdot(T + t)$.
%It is worth noticing that the burst of the output arrival curve at a given node increases due to the experienced delay at the upstream of that node, which is similar to propagating a jitter to account for interferences due to other flows in Scheduling Theory.
%Afterwards, to extend this result to a \textit{network of nodes}, we use the following theorem.
%\begin{Theorem} (Concatenation-Pay Bursts Only Once)
%\label{thm:concat}
%Assume a flow crossing two servers with respective service curves  $\beta_1$ and $\beta_2$. The system composed of the concatenation of the two servers offers a minimum service curve $\beta_1 \otimes \beta_2$ to the flow.
%\end{Theorem}
%
%As an example, for a tandem of nodes with rate-latency service curves, the end-to-end service curve computed according to Th. \ref{thm:concat} is also a rate-latency curve, where the rate is the minimum of the crossed node rates and the latency is the sum of their latencies.
%

Finally, we need the following results concerning the end-to-end service curve of a flow of interest (\emph{foi}) accounting for flows serialization effects in feed-forward networks, based on the Pay Multiplexing Only Once (PMOO) principle \cite{schmitt_pmoo}, under non-preemptive Fixed Priority (FP) multiplexing.


\begin{Theorem}
The service curve offered to a flow of interest $f$ along its path $\path_f$, in a network under non-preemptive FP multiplexing with strict service curve nodes of the rate-latency type $\beta_{R,T}$ and leaky bucket constrained arrival curves $\alpha_{\sigma, \rho}$, is a rate-latency curve, with a rate $R^{\mathbb{P}_f}$ and a latency $T^{\mathbb{P}_f}$, as follows :
%============================================================================
\label{Th:pmoo_fp}
\begin{subequations}
\label{pmoo_fp}
\begin{align}
&  R^{\mathbb{P}_f} = \min \limits_{k \in \mathbb{P}_f} \left( R^{k} - \sum \limits_{i \ni k, i \in shp(f)}{\rho_i} \right) \label{eq:pmoo_fp_R}\\
& T^{\mathbb{P}_f} =  \sum\limits_{k \in \mathbb{P}_f}  \left( T^{k} + \frac{\max\limits_{i \ni k, i \in slp(f)} L_i }{R^k}  \right) \nonumber \\
& + \sum\limits_{i \in DB_{f} \cap shp(f)} \frac{\sigma_i^{\conv(\path_i,\path_f)} + \rho_i \cdot \sum\limits_{k \in\mathbb{P}_f\cap \mathbb{P}_i} \left( T^{k} + \frac{\max\limits_{i \ni k, i \in slp(f)} L_i }{R^k} \right)    } {R^{\mathbb{P}_f}}  \label{eq:pmoo_fp_T}
\end{align}
\end{subequations}
where the required notations are defined in Table \ref{tab:notations}.
%where $slp(f)$ (resp. $shp(f)$) denotes all flows with a priority lower (resp. higher) or equal than $f$ and $L_f$ the maximal packet size of flow $f$.
\end{Theorem}


==> preliminaries.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Buffer-Aware Analysis of Indirect Blocking Traffic
%  \label{sec:preliminaries}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

This section presents a high-level view of the proposed timing analysis.
First, we mention the main steps of the timing analysis. 
Then we recall the approach we developped in \cite{giroudot_buffer_aware}, that we refer to as ``RTAS18 approach'' from now on, on an example. Further details can be found in \cite{giroudot_buffer_aware}.
This approach is valid under the assumption that two packets of the same flow cannot be queueing one right behind the other. 
Finally, we stress out the differences and new aspects of the interference graph approach that will be developped in the next section. 
%This is a direct consequence of the configuration being schedulable. This schedulability assumption is used in \cite{burns_priority_share} as the hypothesis of Theorem 1. %<++>

\subsection{Main Steps of Timing Analysis}
\label{subsec:main_steps}

The main steps of the analysis are similar to our RTAS18 approach. 
To get a bound on the end-to-end latency for a flow $f$, we first need to compute its end-to-end service curve.
As explained in \cite{giroudot_buffer_aware}, the end-to-end service curve of $f$ is denoted :
\[ \beta_{f}(t) = R_f \left( t - T_f \right)^+ \]

And we have :
\begin{equation}
\label{Tf}
T_f = T_{DB} + T_{IB} + T_{\path_f}
\end{equation}
where :
\begin{itemize}
    \item $T_{\path_f}$ is the ``base latency'', that any flit of $f$ experiences along its path due only to the technological latencies of the crossed routers;
    \item $T_{DB}$ is the maximum direct latency, due to interference by flows sharing resources with the flow of interest ;
    \item $T_{IB}$ is the maximum indirect blocking latency, due to flows that can indirectly block $f$ through the buffer backpressure phenomenon.%, and these flows are denoted \textit{indirect blocking} set $IB_f$.
\end{itemize}

In the case of a Fixed-Priority Arbitration between VCs, we denote $T_{DB}$ as :
\[ T_{DB} = T_{hp} + T_{sp} + T_{lp} \]
\begin{itemize}
    \item $T_{hp}$ is part of the maximum direct blocking latency, due to flows of higher priority sharing resources with $f$, which are part of the \textit{direct blocking} set $DB_f$;
    \item $T_{sp}$ is part of the maximum direct blocking latency, due to same priority flows sharing resources with $f$, and also part of $DB_f$ set;
    \item $T_{lp}$ is part of the maximum direct blocking latency, due to flows of lower priority sharing resources with $f$, and also part of $DB_f$ set;
\end{itemize}


We define the indirect blocking set of a flow $f$ as flows that do not physically share any resource with the \emph{foi}, but can delay it because they impact (directly or indirectly) at least one flow of $DB_f$. It is worth noticing that this definition is slightly different from the one used in the Scheduling Theory approaches \cite{burns_priority_share} \cite{liu_tighter_time_analysis}, where there is a distinction between the indirect blocking, due to same-priority flows, and indirect interference, due to higher priority flows. In our approach, we only consider flows belonging to the same class as the \emph{foi} to compute the indirect blocking set, since the impact of higher priority flows is already integrated in our model as follows:

\begin{itemize}
    \item if a higher priority flow blocking our \emph{foi} gets blocked, the \emph{foi} can bypass it. In this case, we take into account the extra processing delay needed to allocate the shared resource to the \emph{foi}. On the other hand, the buffer backpressure will only propagate among flows from the same class, as illustrated in Figure \ref{fig:bypass};
    \item the influence of higher priority flows on the same priority flows than the \emph{foi}, which are inducing the indirect blocking, is modeled through the granted end-to-end service curve of each one of these flows at the rate and latency levels, as explained in Section \ref{subsec:end_to_end_service}
     %indirectly-blocking same priority flows is taken into account through the use of residual service curves. 
\end{itemize}
%ADDED
{\color{blue}
For now, we remain oblivious of how to use the indirect blocking set to derive the corresponding latency. This aspect will be covered in Section \ref{subsec:end_to_end_service}. 
}

To compute the end-to-end latency for the \emph{foi}, we proceed as follows :
\begin{enumerate}
    \item We compute $T_{\path_f}$, then $T_{sp} + T_{hp} + T_{lp}$ using the theorems we recall hereafter ;
    \item We run our indirect blocking analysis and extract the IB set ;
    \item We compute $T_{IB}$. 
    \item From there on, we know the end-to-end service curve for $f$. Thus all that is left is to compute the end-to-end delay bound using Theorem \ref{TH1} :
\begin{equation}
\label{eed}
D_f^{\path_f} = \frac{\sigma^{\path_f[0]}}{R_f} + T_{hp} + T_{sp} + T_{lp} + T_{IB} + T_{\path_f} 
\end{equation}
where $\sigma^{\path_f[0]}$ is the burst of the initial arrival curve of $f$ (the arrival curve of $f$ at node $\path_f[0]$, \ie{} the first node of its path).
\end{enumerate}


The key element to compute the IB set of a flow relies on how packets can spread in the network when stalled.  
Let's consider an intuitive example to better understand the impact of the buffer size on the packet spreading, and consequently the indirect blocking set (Figure \ref{fig:ib_example}).  
We make the following assumptions: (i) each buffer can store only one flit; (ii) all flows have 3-flit-long packets; (iii) all flows are mapped to the same VC; (iv) the \emph{foi} is flow 1.

In the upper configuration, a packet of flow 3 occupies buffers (7, 8, 9). Consequently, a packet of flow 2, waiting for buffer 7, is blocked and occupies buffers (4, 5, 6). In turns, a packet of the \emph{foi} flow 1 is blocked, since it needs buffer 4 to move forward. Hence, flow 3 is included in the indirect blocking set of flow 1. 

In the bottom configuration, a packet of flow 4 occupying buffers (12, 13, 14) leads to a direct blocking of a packet of flow 2, waiting in buffers (7, 8, 11). However, this packet of flow 2 is too far away from the last node flows 1 and 2 have in common (buffer 4). 
%ADDED
{\color{blue}
Provided there is no additional packet of flow 2 stalled right behind the first one, there will be no blocking of flow 1.
}
Hence, flow 4 is not part of the indirect blocking set of the \emph{foi} flow 1, even though there is an intermediate flow that shares resources with both flows 1 and 4.

It is worth noticing that the indirect blocking set analysis without taking into account the buffer size will include flows 3 and 4 in $IB_1 $ (the indirect blocking set of the \emph{foi} flow 1). However, as illustrated in the Figure \ref{fig:ib_example}, there is actually only flow 3 in the indirect blocking set of the \emph{foi} flow 1, due to the impact of the buffer size on the packet spreading. 

%===================================================================================
\begin{figure}[ht]
\centering
\resizebox{1.3\figurewidth}{!}{\input{NC_model_ib_example_1.pdf_tex}} \\
%\rule{0pt}{0pt}\\
\resizebox{1.3\figurewidth}{!}{\input{NC_model_ib_example_2.pdf_tex}}
\caption{Impact of packet size and buffer size on indirect blocking}
\label{fig:ib_example}
\end{figure}
%===================================================================================

Hence, the limited buffer size reduces the section of the path on which a blocked packet can in its turn block another one. 
Consider $k$ and $l$ two flows that are directly interfering with one another, $\path_k, \path_l$ their paths, and let $\dv(\path_k, \path_l)$ be the last node they share :
\[ \dv(\path_k, \path_l) = \path_k[ \max \{i, \path_k[i] \in \path_l \}] \]
Suppose the path of $l$ continues after this node. Even if the head flit of $l$ is not stored in a router of $\path_{k} \cap \path_{l}$, the limited buffer size available in each router can lead to storing the tail flit of $l$ in a router of $\path_{k} \cap \path_{l}$ under contention. In that case, $l$ blocks $k$.

%However, we do have $\path_l[Last_l^k] = \path_k[Last_k^l] = \dv(k,l)$.
Therefore, we need to quantify the way a packet of flow $f$ spreads into the network when it is blocked and stored in buffers :
% Definition : spread index
\begin{Definition}
Consider a flow $f$ of maximum packet length  $L_{f}$ flits, and $B$ the buffer size of a VC in routers, in flits (supposed to be identical for all routers).
The spread index of $f$, denoted $N_{f}$, is defined as follows: 
\[ N_f = \left\lceil \frac{L_{f}}{B} \right\rceil \]
\label{def:spread_index}
\end{Definition}
$N_{f}$ is the number of buffers needed to store one packet of flow $f$.

Using this notion and the last intuitive example, we call the section of the path of flow $k$ from $\dv(\path_k, \path_l)$ to $N_k$ nodes (at most) after $\dv(\path_k, path_l)$ ``subpath of $k$ relatively to $l$'' :
\begin{Definition}
The subpath of a flow $k$ relatively to a flow $l$ is:
\[ subpath(\path_k, \path_l) = \left[ \path_k[Last(\path_k,\path_l) + 1 ], \dots, \path_k[Last(\path_k,\path_l) + N_l] \right] \]
where $Last(\path_k,\path_l) = \max\{ n, \; \path_k[n] \in \path_l\}$ is the index of the last node shared by $k$ and $l$ along $\path_k$, i.e $\path_k[Last(k,l)] = \dv(k,l)$. 
\label{def:subpath1}
\end{Definition}

We can extend this notion and define, in a similar fashion, the subpath of any flow $k$ relatively to a subpath $\subpath_l \subset \path_l$ of any flow $l$ (with $l\neq k$ or $n=k$).
The previous notation still holds :
\begin{Definition}
The subpath of a flow $k$ relatively to any subpath $\subpath_l$ of any flow $l$ is:
\[ subpath(\path_k, \subpath_l) = \left[ \path_k[Last(\path_k, \subpath_l) + 1 ], \dots, \path_k[Last(\path_k, \subpath_l) + N_l] \right] \]
where $Last(\path_k,\subpath_l) = \max\{ n, \; \path_k[n] \in \subpath_l\}$ is the index along $\path_k$ of the last node shared by $k$ on $\path_k$ and $l$ restricted to $\subpath_l$.
By abuse of notation, we may denote $subpath(k,l)$ to refer to $subpath(\path_k,\path_l)$, and similarly $subpath(k, \subpath_l)$ to refer to $subpath(\path_k,\subpath_l)$.
\end{Definition}


It is worth noticing that if $\path_l$ ends before reaching the $N_l$-th node after $\dv(k,l)$, then we ignore the out-of-range indexes. The notion of subpath is illustrated in Figure \ref{fig:subpath} for the \emph{foi} $k$ and a spread index for the interfering flow $l$ equal to 3, \ie{}, $N_l =3$.

\begin{figure}[ht]
\centering
\resizebox{\figurewidth}{!}{\input{NC_model_subpath.pdf_tex}}
\caption{Subpath illustration for the \emph{foi} $k$}
\label{fig:subpath}
\end{figure}




\subsection{Recap of RTAS18 Approach}

Hereafter, %we recall notions introduced in our previous approach. Then 
we detail the computation of the indirect blocking set $IB_f$, as first presented in \cite{giroudot_buffer_aware}, on an example. 
We then recall the way we compute $T_{IB}$ using the computed IB set. 

%To better understand the impact of the buffer size on the packet spreading, and consequently the indirect blocking set, we consider the example of Figure \ref{fig:ib_example} under the following assumptions: (i) each buffer can store only one flit; (ii) all flows have 3-flit-long packets; (iii) all flows are mapped to the same VC; (iv) the \emph{foi} is flow 1.
%
%In the upper configuration, a packet of flow 3 occupies buffers (7, 8, 9). Consequently, a packet of flow 2, waiting for buffer 7, is blocked and occupies buffers (4, 5, 6). In turns, a packet of the \emph{foi} flow 1 is blocked, since it needs buffer 4 to move forward. Hence, flow 3 is included in the indirect blocking set of the \emph{foi} flow 1. 
%
%In the bottom configuration, a packet of flow 4 occupying buffers (12, 13, 14) leads to a direct blocking of a packet of flow 2, waiting in buffers (7, 8, 11). However, this packet of flow 2 is too far away from the last node flows 1 and 2 have in common (buffer 4). 
%%ADDED
%{\color{blue}
%Provided there is no additional packet of flow 2 stalled right behind the first one, there will be no blocking of flow 1.
%}
%Hence, flow 4 is not part of the indirect blocking set of the \emph{foi} flow 1, even though there is an intermediate flow that shares resources with both flows 1 and 4.
%
%It is worth noticing that the indirect blocking set analysis without taking into account the buffer size will include flows 3 and 4 in $IB_1 $ (the indirect blocking set of the \emph{foi} flow 1). However, as illustrated in the Figure \ref{fig:ib_example}, there is actually only flow 3 in the indirect blocking set of the \emph{foi} flow 1, due to the impact of the buffer size on the packet spreading. 
%
%
%
%%===================================================================================
%\begin{figure}[ht]
%\centering
%\resizebox{1.3\figurewidth}{!}{\input{NC_model_ib_example_1.pdf_tex}} \\
%%\rule{0pt}{0pt}\\
%\resizebox{1.3\figurewidth}{!}{\input{NC_model_ib_example_2.pdf_tex}}
%\caption{Impact of packet size and buffer size on indirect blocking}
%\label{fig:ib_example}
%\end{figure}
%%===================================================================================
%
%Hence, the limited buffer size reduces the section of the path on which a blocked packet can in its turn block another one. 
%Consider $k$ and $l$ two flows that are directly interfering with one another, $\path_k, \path_l$ their paths, and let $\dv(\path_k, \path_l)$ be the last node they share :
%\[ \dv(\path_k, \path_l) = \path_k[ \max \{i, \path_k[i] \in \path_l \}] \]
%Suppose the path of $l$ continues after this node. Even if the head flit of $l$ is not stored in a router of $\path_{k} \cap \path_{l}$, the limited buffer size available in each router can lead to storing the tail flit of $l$ in a router of $\path_{k} \cap \path_{l}$ under contention. In that case, $l$ blocks $k$.
%
%%However, we do have $\path_l[Last_l^k] = \path_k[Last_k^l] = \dv(k,l)$.
%Therefore, we need to quantify the way a packet of flow $f$ spreads into the network when it is blocked and stored in buffers. 
%%<++>
%We do so by computing $N_{f}$, the number of buffers needed to store one packet of flow $f$. We call $N_f$ the ``spread index for flow $f$''.
%Given the maximum packet length of flow $f$, $L_{f}$ flits, and the buffer size of a VC in routers $B$ flits (supposed to be identical for all routers), $N_{f}$ verifies : 
%\[ N_f = \left\lceil \frac{L_{f}}{B} \right\rceil \]
%%It is worth noticing that we use the flit as a unit for packet length and buffer size.
%
%
%Using the previous example, we call the section of the path of flow $l$ from $\dv(\path_k, \path_l)$ to $N_k$ nodes (at most) after $\dv(\path_k, path_l)$ ``subpath of $k$ relatively to $l$'' :
%\[ subpath(\path_k, \path_l) = \left[ \path_k[Last(\path_k,\path_l) + 1 ], \dots, \path_k[Last(\path_k,\path_l) + N_l] \right] \]
%where $Last(\path_k,\path_l) = \max\{ n, \; \path_k[n] \in \path_l\}$ is the index of the last node shared by $k$ and $l$ along $\path_k$, i.e $\path_k[Last(k,l)] = \dv(k,l)$. 
%
%
%We can extend this notion and define, in a similar fashion, the subpath of any flow $k$ relatively to a subpath $\subpath_l \subset \path_l$ of any flow $l$ (with $l\neq k$ or $n=k$).
%The previous notation still holds :
%\[ subpath(\path_k, \subpath_l) = \left[ \path_k[Last(\path_k, \subpath_l) + 1 ], \dots, \path_k[Last(\path_k, \subpath_l) + N_l] \right] \]
%where $Last(\path_k,\subpath_l) = \max\{ n, \; \path_k[n] \in \subpath_l\}$ is the index along $\path_k$ of the last node shared by $k$ on $\path_k$ and $l$ restricted to $\subpath_l$.
%
%
%It is worth noticing that if $\path_l$ ends before reaching the $N_l$-th node after $\dv(k,l)$, then we ignore the out-of-range indexes. The notion of subpath is illustrated in Figure \ref{fig:subpath} for the \emph{foi} $k$ and a spread index for the interfering flow $l$ equal to 3, \ie{}, $N_l =3$.
%
%By abuse of notation, we may denote $subpath(k,l)$ to refer to $subpath(\path_k,\path_l)$,
%and similarly $subpath(k, \subpath_l)$ to refer to $subpath(\path_k,\subpath_l)$.
%%======================================================================================================================
%\begin{figure}[ht]
%\centering
%\resizebox{\figurewidth}{!}{\input{NC_model_subpath.pdf_tex}}
%\caption{Subpath illustration for the \emph{foi} $k$}
%\label{fig:subpath}
%\end{figure}
%%=================================================


%We also need the following definitions :
We will need the following definitions :
\begin{itemize}
  \item $sp(f)$: all flows belonging to the same VC as $f$, $f$ excluded ;
  \item $hp(f)$: all flows mapped to a VC of strict higher priority than the VC, to which $f$ belongs;
  \item $lp(f)$: all flows mapped to a VC of strict lower priority than the VC, to which $f$ belongs;
  \item $DB_f $: set of all flows directly interfering with flow $f$, regardless of their priority, \ie{}, $DB_f = \{ i \in \mathcal{F}, \; \path_i \cap \path_f \neq \varnothing \}$;
  \item $DB_f^{|path}$: set of flows of $DB_f$ with paths having a non-null intersection with $path \subset \path_f$, \ie{} $DB_f^{|path} = \{ i \in DB_f$, \; $\path_i \cap path \neq \varnothing \}$.
\end{itemize}


The main steps of the RTAS18 algorithm to determine the IB set a flow $f$ are as follows:
\begin{enumerate}
    \item determine all subpaths of flows in $DB_f^{|\path_f} \cap sp(f)$ relatively to flow $f$;
    \item for each of these subpaths, check if they intersect with other flows. If yes, determine the subpaths of these other flows relatively to the subpath they intersect;
    \item add the new found subpaths to the set and reiterate until no new subpath is found. 
\end{enumerate}
%The function call ${\rm computeDBset}(j,path)$ returns all the flows of $DB_j^{|path} \cap sp(j)$ and their associated subpath relatively to $j$. 
Notice that no flow can be found both in $DB_f \cap sp(f)$ and in $IB_f$, since the influence of directly-interfering, same-priority flows is already integrated through the computation of the direct blocking latency, which will be detailed in Section \ref{subsec:end_to_end_service}.
Moreover, this algorithm can be used to compute the subset of $IB_f$ containing only flows that can cause indirect blocking on a subpath $subP \subset \path_f$. In that case, we need to consider $DB_f^{|subP}$ instead of $DB_f$, and we will note the result "partial indirect blocking set" $IB_f^{|subP}$. 

We can also choose to ignore a subset of the flows in $\mathcal{F}$ during the algorithm, using an optional parameter. 
We can put in this subset the flows that we have already taken into account before. For instance, when we compute the impact of a flow $i$ on the \emph{foi} $f$, we must exclude flow $f$ from the flows impacting flow $i$. In fact, if not doing so, it would be equivalent to consider that flow $f$ impacts itself, which is quite pessimistic.


%\begin{algorithm}
%\caption{Determining $IB_f$ and the associated subpaths}
%\label{alg:ib}
%%indirectBlockingSet($f$, $\path_f$, toIgnore)
%\begin{algorithmic}[1]
%    \REQUIRE{$f$, the flow of interest, $\path_f$ the associated path, toIgnore a list of flows to ignore (optional)}
%    \ENSURE{$IB_f$, a set containing flow indexes and associated subpath involved in indirect interference on $\path_f$}
%    \STATE $IB_f$ is initially empty
%    \STATE $init\_set \leftarrow DB_f^{|\path_f} \cap sp(f)$ \\
%    {\color{darkgreen}\COMMENT{ initialize $S$ }}%-- contains flow indexes and associated subpath to be treated :}}
%    \FOR{$i \in init\_set \backslash {\rm toIgnore}$} \label{lin:init_start}
%        \STATE Append $\{i,i.{\rm subpath}(f)\}$ to $S$ 
%    \ENDFOR \label{lin:init_end}
%
%    %\STATE ${\rm processedFlows} \leftarrow \varnothing$ {\color{darkgreen}\COMMENT{ Initialize processedFlows }}%-- contains indexes of processed flows :}} 
%    \WHILE{$S \neq \varnothing$}
%        \STATE Pop a pair $\{ j, {\rm subj}\}$ from $S$ \\
%        %\STATE $g \leftarrow$ Flow($j$, sub) {\color{darkgreen}\COMMENT{ create a fake flow with same parameters as $j$ except the path}} \\
%        {\color{darkgreen}\COMMENT{ Compute subpaths relatively to $j$ on subj :}}
%	\STATE ${\rm currentDB} \leftarrow$ computeDBset($j, {\rm subj}$)  \label{lin:dbtest} %{\color{darkgreen}\COMMENT{ $DB_j^{|subj}$}} 
%        \FOR{($k, {\rm subk}$) $\in {\rm currentDB}\cap sp(j)$}
%            %\IF{$k \in {\rm processedFlows} \cup init\_set \cup {\rm toIgnore}$} \label{lin:test}
%            %    \STATE Move directly to the next iteration of the loop
%            %\ENDIF
%	\IF{$(k,{\rm subk}) \notin IB_f$}
%                \STATE Append $(k,{\rm subk})$ to $IB_f$ and $S$ \label{lin:add}
%            \ENDIF
%        \ENDFOR
%        %\STATE Append $j$ to processedFlows
%    \ENDWHILE \label{lin:end}
%    \RETURN{$IB_f$}
%\end{algorithmic}
%\end{algorithm}

\begin{application}
    An application of the algorithm to compute $IB_f$ is illustrated in Figure \ref{fig:contention}, when considering the flow $f$ as the \emph{foi} and four more flows with the same priority as $f$ and a spread index of 3.  
    First, the algorithm will initialize the set $S$ with flow indexes and subpaths from $DB_f$ :\\
    \[ S = \left\{ \{1, S_1\}, \{2, S_2\} \right\} \] 
    Then, we enter the while loop : 
    \begin{enumerate}
      \item we pop $\{1, S_1\}$ and check if it does not intersect any other flow : ${\rm currentDB} = \varnothing$. We add 1 to processedFlows. $S$ now contains $\{2, S_2\}$. 
      \item we pop $\{2, S_2\}$ and compute ${\rm currentDB} = \left\{ 3, S_3 \right\}$. We add $\{3,S_3\}$ to $IB_f$ and to $S$. We add 2 to processedFlows. $S$ now contains $\{3, S_3\}$. 
      \item we pop $\{3, S_3\}$ and compute ${\rm currentDB} = \left\{ 4, S_4 \right\}$. We add $\{4,S_4\}$ to $IB_f$ and $S$. We add 3 to processedFlows. $S$ now contains $\{4, S_4\}$;
      \item we pop $\{4, S_4\}$ and compute ${\rm currentDB} = \varnothing$. We add 4 to processedFlows. $S$ is now empty, the loop is over.
    \end{enumerate}
    Thus, we finally have :
    \[ IB_f = \left\{ \{3, S_3\}, \{4, S_4\} \right\} \]
\end{application}
%===================================================================================
\begin{figure}[ht]
\centering
\resizebox{\figurewidth}{!}{\input{NC_model_contending_flows_example.pdf_tex}}
\caption{Several contending flows and the subpaths with $f$ as the flow of interest. Green : subpaths included in $IB_f$ after the algorithm ; red : subpaths of $DB_f$.}
\label{fig:contention}
\end{figure}
%=================================================================================== 

We compute $T_{IB}$ as follows :
\begin{equation}
\label{indirectBlocking}
T_{IB} = \sum_{\{k,subP\} \in IB_f} \frac{\sigma_k^{subP[0]} }{\widetilde{R}_k^{subP} } + \widetilde{T}_k^{subP}
\end{equation}

where:
\begin{subequations}
\label{eq:vc_scurve}
\begin{align}
& \widetilde{R}_k^{subP} =  \min\limits_{r \in subP} \left\{ R^r - \sum\limits_{j \ni r, j \in hp(f)} \rho_j \right\} \label{eq:vc_scurve_R}  \\
& \widetilde{T}_k^{subP} =  \sum\limits_{r \in subP} \left( T^r 
                                        +  \frac{S_{flit} \mathbf{1}_{ \{lp(k) \supset r\}} }
                                                 {R^{r}} \right) \nonumber \\
& +      \sum\limits_{i \in DB_k^{|subP} \cap hp(k)} \frac{\sigma_i^{\conv(i,k)} + 
           \rho_i \sum\limits_{r \in subP \cap \path_i} 
           \left( T^r + \frac{S_{flit} \mathbf{1}_{\{lp(k) \supset r\}} }{R^{r}} \right) }{\widetilde{R}_k^{subP}} \label{eq:vc_scurve_T} 
\end{align}
\end{subequations}

For each pair \{flow, subpath\} in the IB set, we have to compute the arrival curve of the flow at the beginning of the subpath, as the burst of the said arrival curve (denoted $\sigma_k^{subP[0]}$) is used to compute $T_{IB}$.

\subsection{Novelties of Interference Graph Approach}

The new approach we introduce in the next section presents several improvements to RTAS18 method. 
First, extending interference notions, it applies to architectures with heterogeneous buffer sizes.
Second, it does not rely on any assumption regarding the backlogged period of flows. This ensures computed bounds are allways safe.
Third, the computation of $T_{IB}$ is done without propagating the arrival curve of each flow at the beginning of its subpath. We will detail this aspect in Section \ref{subsec:end_to_end_service}.

Figure \ref{fig:comparative_approach} sums up the main differences between the two approaches in the end-to-end latency computing process.

\begin{figure}[ht]
\centering
\resizebox{\figurewidth}{!}{\input{NC_model_approach_comparative_synthesis.pdf_tex}}
\caption{Computing end-to-end service curve latency : comparative of RTAS18 and GRAPH approach.}
\label{fig:comparative_approach}
\end{figure}


==> recap_rtas18_approach.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Recap of BATA approach
%  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

This section recaps our previously-published timing-analysis approach, BATA.
We detail the computation of the IB set, then of the corresponding indirect blocking latency. 
We illustrate these steps on an example.

\subsection{Computing IB Set}

The main steps of the algorithm to determine the IB set for a flow $f$ are as follows:
\begin{enumerate}
    \item determine all subpaths of flows in $DB_f^{|\path_f} \cap sp(f)$ relatively to flow $f$;
    \item for each of these subpaths, check if they intersect with other flows. If yes, determine the subpaths of these other flows relatively to the subpath they intersect;
    \item add the new found subpaths to the set and reiterate until no new subpath is found. 
\end{enumerate}

Notice that flows in $DB_f \cap sp(f)$ have no subpath in $IB_f$, since the influence of directly-interfering, same-priority flows is already integrated through the computation of the direct blocking latency.
Moreover, this algorithm can be used to compute the subset of $IB_f$ containing only flows that can cause indirect blocking on a subpath $subP \subset \path_f$. In that case, we need to consider $DB_f^{|subP}$ instead of $DB_f$, and we will note the result "partial indirect blocking set" $IB_f^{|subP}$. 
We present the detailed algorithm hereafter (\ref{alg:ib}). 

\begin{algorithm}
\caption{Determining $IB_f$ and the associated subpaths}
\label{alg:ib}
%indirectBlockingSet($f$, $\path_f$, toIgnore)
\begin{algorithmic}[1]
    \REQUIRE{$f$, the flow of interest, $\path_f$ the associated path, toIgnore a list of flows to ignore (optional)}
    \ENSURE{$IB_f$, a set containing flow indexes and associated subpath involved in indirect interference on $\path_f$}
    \STATE $IB_f$ is initially empty
    \STATE $init\_set \leftarrow DB_f^{|\path_f} \cap sp(f)$ \\
    {\color{darkgreen}\COMMENT{ initialize $S$ }}%-- contains flow indexes and associated subpath to be treated :}}
    \FOR{$i \in init\_set \backslash {\rm toIgnore}$} \label{lin:init_start}
        \STATE Append $\{i,i.{\rm subpath}(f)\}$ to $S$ 
    \ENDFOR \label{lin:init_end}

    %\STATE ${\rm processedFlows} \leftarrow \varnothing$ {\color{darkgreen}\COMMENT{ Initialize processedFlows }}%-- contains indexes of processed flows :}} 
    \WHILE{$S \neq \varnothing$}
        \STATE Pop a pair $\{ j, {\rm subj}\}$ from $S$ \\
        %\STATE $g \leftarrow$ Flow($j$, sub) {\color{darkgreen}\COMMENT{ create a fake flow with same parameters as $j$ except the path}} \\
        {\color{darkgreen}\COMMENT{ Compute subpaths relatively to $j$ on subj :}}
	\STATE ${\rm currentDB} \leftarrow$ computeDBset($j, {\rm subj}$)  \label{lin:dbtest} %{\color{darkgreen}\COMMENT{ $DB_j^{|subj}$}} 
        \FOR{($k, {\rm subk}$) $\in {\rm currentDB}\cap sp(j)$}
            %\IF{$k \in {\rm processedFlows} \cup init\_set \cup {\rm toIgnore}$} \label{lin:test}
            %    \STATE Move directly to the next iteration of the loop
            %\ENDIF
	\IF{$(k,{\rm subk}) \notin IB_f$}
                \STATE Append $(k,{\rm subk})$ to $IB_f$ and $S$ \label{lin:add}
            \ENDIF
        \ENDFOR
        %\STATE Append $j$ to processedFlows
    \ENDWHILE \label{lin:end}
    \RETURN{$IB_f$}
\end{algorithmic}
\end{algorithm}

%The complexity of Algorithm \ref{alg:ib} is $ $. 

\begin{application}
	Applying Algorithm \ref{alg:ib} on the configuration of Figure \ref{fig:intuitive_example_config} (recalled on Figure \ref{fig:subpath_computation_example}) with flow 1 as the \emph{foi} and assuming all flows have a spread index of 3, we proceed as follow :
\begin{enumerate}
	\item We check for flows intersecting flow 1 path. There is only flow 2, so we compute its subpath relatively to flow 1, that we denote $\subpath_a$.
	\item We check for intersection between $\subpath_a$ and other paths. Flow 3 intersects $\subpath_a$, so we compute its subpath relatively to $\subpath_a$ and we add it to $IB_1$. We denote it $\subpath_b$.
	\item We check intersections with $\subpath_b$ and find that there are none. The algorithm stops.
\end{enumerate}
The result is shown on Figure \ref{fig:subpath_computation_example}
We finally have :
\[ IB_1 = \left\{ \{3,\subpath_b\} \right\}  \]
\begin{figure}[ht]
    \centering
    \resizebox{0.5\columnwidth}{!}{\input{WIP_intuitive_example.pdf_tex}}\resizebox{0.5\columnwidth}{!}{\input{WIP_intuitive_example_subpaths.pdf_tex}}
    \caption{Example configuration (left) and subpath computation (right)}
    \label{fig:subpath_computation_example}
\end{figure}
\end{application}

\subsection{Indirect Blocking Latency Computation}

Knowing the IB set, we compute the maximum indirect blocking latency with the following Theorem.

\begin{Theorem}
\label{Th:indirectblocking}(Maximum Indirect Blocking Latency)\\
The maximum indirect blocking latency for a \emph{foi} $f$ along its path $\path_f$, in a NoC under flit-level preemptive FP multiplexing with strict service curve nodes of the rate-latency type $\beta_{R,T}$ and leaky bucket constrained arrival curves $\alpha_{\sigma, \rho}$, is as follows:
%========================================================================================================================================================
\begin{equation}
\label{indirectBlocking}
T_{IB} = \sum_{(k,subP) \in IB_f} \frac{\sigma_k^{subP[0]} }{\widetilde{R}_k^{subP} } + \widetilde{T}_k^{subP}
\end{equation}

where:
\begin{subequations}
\label{eq:vc_scurve}
\begin{align} 
& \widetilde{R}_k^{subP} =  \min\limits_{r \in subP} \left\{ R^r - \sum\limits_{j \ni r, j \in hp(f)} \rho_j \right\} \label{eq:vc_scurve_R}  \\
& \widetilde{T}_k^{subP} =  \sum\limits_{r \in subP} \left( T^r 
                                        +  \frac{S_{flit} \mathbf{1}_{ \{lp(k) \supset r\}} }
                                                 {R^{r}} \right) + \nonumber \\
&  \sum\limits_{i \in DB_k^{|subP} \cap hp(k)} \frac{\sigma_i^{\conv(i,k)} + 
           \rho_i \sum\limits_{r \in subP \cap \path_i} 
           \left( T^r + \frac{S_{flit} \mathbf{1}_{\{lp(k) \supset r\}} }{R^{r}} \right) }{\widetilde{R}_k^{subP}} \label{eq:vc_scurve_T} 
\end{align}
\end{subequations}
\end{Theorem}
Once again, the proof can be found in \cite{giroudot_buffer_aware}.
Computing $T_{IB}$ with this theorem may lead to recursive computations of end-to-end service curves. We illustrate this in the following application.

\begin{application}
    To compute the indirect blocking latency for flow 1 on the configuration of Figure \ref{fig:intuitive_example_config}, we need to compute the arrival curve of flow 3 at R7 (more precisely we're interested in the burst of this flow at the input of R7).
    This leads to recursive calls. 	
    % For this, we need to know the service curve granted to flow 3 on [R6]. 
    % For this, we compute the (partial) maximum direct blocking latency for flow 3 using Theorem \ref{Th:indirectblocking}.
    % We thus need to compute the burst of flow 2 R6, for which we need the partial service curve granted to flow 2 on [R3, R4, R5].
    % Finally 
    
    \noindent The service curve granted to flow 1 on [R1, R2] is:
    \[\beta_1^{[R1, R2]} = R(t - 2T)^+\]
    The burst of flow 1 at R3 is thus 
    \[\sigma_1^{R3} = \sigma + 2 \rho T\]
    The service curve granted to flow 2 on [R3, R4, R5] is:
    \[\beta_2^{[R3, R4, R5]} = (R-\rho) \left( t - 3T - \frac{ \sigma_1^{R3} + \rho (T + \frac{L}{R})}{R - \rho} \right)^+\]
    The burst of flow 2 at R6 is thus:
    \[\sigma_2^{R6} = \sigma + \rho \left( 3T + \frac{ \sigma_1^{R3} + \rho (T + \frac{L}{R})}{R - \rho} \right)\]
    The service curve granted to flow 3 on [R6] is:
    \[\beta_3^{[R6]} = (R - \rho) \left( t - T - \frac{ \sigma_2^{R6} + \rho (T + \frac{L}{R})}{R - \rho} \right)^+\]
    Finally, the burst of flow 3 at R7 is:
    \[ \sigma_3^{R6} = \sigma + \rho \left( T + \frac{ \sigma_2^{R6} + \rho (T + \frac{L}{R})}{R - \rho} \right) \]

    Numerically, with $R = 1$ flit/cycle, $T = 1$ cycle, $\rho = 0.05$ flits/cycle, $\sigma = 3$ flits and $L = 3$ flits, we have :
    \begin{eqnarray*}
    	\sigma_1^{R3} &=& 3 + 2 \times 0.05 \times 1\\
    	              &=& 3.1 \\
        \sigma_2^{R6} &=& 3 + 0.05 \times \left( 3 \times 1 + \frac{3.1 + 0.05 (1 + 3/1)}{0.95} \right) \\
                      &=& 3 + 0.05 \times \left( 3 + 3.3/0.95 \right) \\
                      &=& 3.323684211 \\
        \sigma_3^{R7} &=& 3 + 0.05 \times \left( 1 + \frac{3.323684211 + 0.05 (1 + 3/1)}{0.95} \right)\\
                    &=& 3 + 0.05 \times \left( 1 + 3.709141275 \right) \\
                    &=& 3.235457064\\
    \end{eqnarray*}
    
    Then we compute $\widetilde{T_3}^{[R7, R8, R9]}$. Since there are no higher or lower priority flows on the configuration, we have :
    \begin{eqnarray*}
        \widetilde{T_3}^{[R7, R8, R9]} &=& 3T \\
        \widetilde{R_3}^{[R7, R8, R9]} &=& R
    \end{eqnarray*}
    Finally:
    \begin{eqnarray*}
    	T_{IB} &=& 3T + \sigma_3^{R7}/R \\
    	       &=& 6.235457064 
    \end{eqnarray*}
    We had to perform 3 additional calls to the function computing the end-to-end service curve.
\end{application}

\subsection{Identified Limitations}

Consider the second example used in Section \ref{subsec:illustrative_example}, recalled on Figure \ref{fig:problematic_example_cpq}. 
When computed with BATA approach, the IB set of flow 1 $IB_1$ is empty because a packet of flow 3 cannot block flow 1. 
However, this relies on the assumption that there is no CPQ. 

To see how this limits the applicability of BATA approach, consider the packet configuration shown on Figure \ref{fig:problematic_example_cpq}. 
As before, a packet A of flow 3 is being transmitted. It requested and was granted output port North of R7. 
Flow 2 has a packet B also requesting output port North of R7 but as A is using it, it has to wait. 
B is stored in buffers in R5, R6 and R7. 
Moreover, there is an additional packet of flow 2, C, right behind B.
It was granted the use of output port East of R3 and is waiting at R4 for the next input buffer of its path to be abailable.
Finally, flow 1 has a packet D requesting the output port East of R3. Since C is already using this output, D has to wait.

Thus, packet D has to wait that packet A releases output port North of R7 to be able to move. 
This means flow 3 can indirectly block flow 1, even though BATA approach did not cover such a scenario. 
\bigskip
\begin{figure}[ht]
     \centering
     \resizebox{0.48\columnwidth}{!}{\input{WIP_problematic_example.pdf_tex}}\resizebox{0.52\columnwidth}{!}{\input{WIP_problematic_example_packet_detail.pdf_tex}}
     \caption{Example configuration (left) and CPQ not taken into account by BATA approach (right)}
     \label{fig:problematic_example_cpq}
\end{figure}

%We thus want to extend BATA model to cover such scenarios. 
%This will be covered in Section \ref{sec:interference_graph_approach}.
To cover the CPQ assumption, we introduce the new Interference Graph approach, referred to as GRAPH, in Section \ref{sec:interference_graph_approach}.


% We can also choose to ignore a subset of the flows in $\mathcal{F}$ during the algorithm, using an optional parameter. 
% We can put in this subset the flows that we have already taken into account before. For instance, when we compute the impact of a flow $i$ on the \emph{foi} $f$, we must exclude flow $f$ from the flows impacting flow $i$. In fact, if not doing so, it would be equivalent to consider that flow $f$ impacts itself, which is quite pessimistic.
% 

% \begin{application}
%     An application of the algorithm to compute $IB_f$ is illustrated in Figure \ref{fig:contention}, when considering the flow $f$ as the \emph{foi} and four more flows with the same priority as $f$ and a spread index of 3.  
%     First, the algorithm will initialize the set $S$ with flow indexes and subpaths from $DB_f$ :\\
%     \[ S = \left\{ \{1, S_1\}, \{2, S_2\} \right\} \] 
%     Then, we enter the while loop : 
%     \begin{enumerate}
%       \item we pop $\{1, S_1\}$ and check if it does not intersect any other flow : ${\rm currentDB} = \varnothing$. We add 1 to processedFlows. $S$ now contains $\{2, S_2\}$. 
%       \item we pop $\{2, S_2\}$ and compute ${\rm currentDB} = \left\{ 3, S_3 \right\}$. We add $\{3,S_3\}$ to $IB_f$ and to $S$. We add 2 to processedFlows. $S$ now contains $\{3, S_3\}$. 
%       \item we pop $\{3, S_3\}$ and compute ${\rm currentDB} = \left\{ 4, S_4 \right\}$. We add $\{4,S_4\}$ to $IB_f$ and $S$. We add 3 to processedFlows. $S$ now contains $\{4, S_4\}$;
%       \item we pop $\{4, S_4\}$ and compute ${\rm currentDB} = \varnothing$. We add 4 to processedFlows. $S$ is now empty, the loop is over.
%     \end{enumerate}
%     Thus, we finally have :
%     \[ IB_f = \left\{ \{3, S_3\}, \{4, S_4\} \right\} \]
% \end{application}
% %===================================================================================
% \begin{figure}[ht]
% \centering
% \resizebox{\figurewidth}{!}{\input{NC_model_contending_flows_example.pdf_tex}}
% \caption{Several contending flows and the subpaths with $f$ as the flow of interest. Green : subpaths included in $IB_f$ after the algorithm ; red : subpaths of $DB_f$.}
% \label{fig:contention}
% \end{figure}
% %=================================================================================== 
% 
% For each pair \{flow, subpath\} in the IB set, we have to compute the arrival curve of the flow at the beginning of the subpath, as the burst of the said arrival curve (denoted $\sigma_k^{subP[0]}$) is used to compute $T_{IB}$.


==> related_work.tex <==

\renewcommand{\arraystretch}{1.0}
\rule{-3cm}{0cm}\begin{table*}
\centering
% \begin{tabular}{@{}lccccccccc@{}}
% \toprule
%                   &                                     & wormhole & multiple VCs & priority sharing & VCs sharing & flows serialization & \multicolumn{3}{@{}c@{}}{buffer size $B$ (\emph{vs} packet length $L$)} \\
% \multicolumn{2}{@{}l@{}}{Contrib.}                      &          &              &                 &           &               & 1 flit & $L \leq B$ & $B \leq L$ \\
% \midrule
%         &\cite{xiong_extending_rt_analysis_nocs}        & \tickx   & \tickx       & \untck          & \untck    & \untck        & \tickx & \tickx     & \tickx     \\
% ST      &\cite{burns_priority_share}                    & \tickx   & \tickx       & \tickx          & \untck    & \untck        & \untck & \untck     & \untck     \\
%         &\cite{liu_tighter_time_analysis}               & \tickx   & \tickx       & \tickx          & \untck    & \untck        & \tickx & \untck     & \untck     \\
% 
% \midrule
% CPA     &\cite{tobuschat_ernst_cpa_noc_backpressure}    & \tickx   & - \untck     & \tickx          & \untck    & \untck        & \untck & \tickx     & \untck     \\
%         &\cite{Rambo:2015:WCT}                          & \tickx   & \tickx       & \tickx          & \tickx    & \untck        & \untck & \tickx     & \untck     \\
% 
% \midrule
%         &\cite{qian_analysis_worst_case_delays_wormhole}& \tickx   & \untck       & \tickx          & \untck    & \untck        & \tickx & \tickx     & \tickx     \\
% NC      &\cite{jafari_ludb_vbr_flows_noc_vc}            & \untck   & \tickx       & \tickx          & \untck    & \tickx        & \untck & \tickx     & \untck     \\
%         &\cite{boyer_computing_routes_kalray}           & \tickx   & \tickx       & \untck          & - \untck  & \tickx        & \untck & \untck & \tickx \\
%         &\textbf{\cite{giroudot_buffer_aware}}          & \textbf{\tickx} & \textbf{\tickx} & \textbf{\tickx} & \textbf{\tickx} & \textbf{\tickx} & \textbf{\tickx} & \textbf{\tickx} & \textbf{\tickx}\\
%         %& \textbf{extended approach \cite{giroudot_buffer_aware}} & \textbf{\tickx}   & \textbf{\tickx}       & \textbf{\tickx}          & \textbf{\tickx}    & \textbf{\tickx}        & \textbf{\tickx} & \textbf{\tickx}     & \textbf{\tickx    } \\
% 
% \bottomrule
% \end{tabular}

\begin{tabular}{@{}l|cccc|cc|cc|ccccc}
\toprule
Approach                      & \multicolumn{4}{c|}{ST} & \multicolumn{2}{c|}{CPA} & \multicolumn{2}{c|}{RC} & \multicolumn{5}{c}{NC} \\
Contribution                  &\cite{xiong_extending_rt_analysis_nocs} &\cite{burns_priority_share} &\cite{liu_tighter_time_analysis} & \cite{nikolic_rt_analysis_priority_preemptive_nocs} &\cite{tobuschat_ernst_cpa_noc_backpressure} &\cite{Rambo:2015:WCT} &\cite{ferrandiz_recursive_calculus} &\cite{liu_buffer_aware} &\cite{qian_analysis_worst_case_delays_wormhole} &\cite{jafari_ludb_vbr_flows_noc_vc} &\cite{boyer_computing_routes_kalray} &\textbf{BATA\cite{giroudot_buffer_aware}} & \textbf{GRAPH}\\
\midrule


wormhole                      & \v     & \v    & \v    & \v    & \v    & \v    & \v    & \v    & \v  & \x  & \v  & \v  & \v  \\
multiple VCs                  & \v     & \v    & \v    & \v    & \x    & \v    & \x    & \x    & \x  & \v  & \v  & \v  & \v  \\
priority sharing              & \x     & \v    & \v    & \x    & \v    & \v    & \x    & \x    & \v  & \v  & \x  & \v  & \v  \\
VCs sharing                   & \x     & \x    & \x    & \x    & \x    & \v    & \x    & \x    & \x  & \x  & \x  & \v  & \v  \\
flows serialization           & \x     & \x    & \x    & \v    & \x    & \v    & \x    & \x    & \x  & \v  & \v  & \v  & \v  \\
$B = $ 1 flit                 & \v     & \x    & \v    & \v    & \x    & \x    & \x    & \v    & \v  & \x  & \x  & \v  & \v  \\
$L \leq B$                    & \v     & \x    & \x    & \v    & \v    & \v    & \x    & \v    & \v  & \v  & \x  & \v  & \v  \\
$B \leq L$                    & \v     & \x    & \x    & \v    & \x    & \x    & \x    & \v    & \v  & \x  & \v  & \v  & \v  \\
support CPQ                   & \nes   & \nes  & \nes  & \nes  & \nes  & \nes  & \nes  & \nes  & \v  & \x  & \v  & \x  & \v  \\
\bottomrule
	
\end{tabular}

\smallskip
\caption{Summary of the assumptions of the main existing approaches : Scheduling Theory (ST), CPA and Network Calculus (NC). ``GRAPH'' refers to our extended approach developped in this paper. \nes : Not Explicitely Specified.}

\label{tab:related_work_summary}
\end{table*}
\renewcommand{\arraystretch}{1.5}
%==============================================================================

Networks-on-Chip (NoCs), and more specifically wormhole NoCs, are the prefered interconnect for complex system-on-chip and manycore architectures. They consist of routers connected with processing elements (or other on-chip components) and other routers in such a way that any component can send a message to another.
There is a great variety of NoCs in terms of topology, routing algorithms and flow control techniques, and an equally diverse panel of timing analysis methods. 

Although many NoC topologies have been proposed and evaluated in the literature \cite{survey_wormhole,kim_flattened_butterfly,dally_kary_ncube}, \emph{low-dimensional topologies} \cite{kavaldjiev2003_survey_onchip_communications} are the most common ones, since  
they exhibit good scalability and energy-efficiency while achieving substantial wiring complexity reduction.
Such topologies include 2D-mesh \cite{wentzlaff_on_chip_interconnection_architecture_tile_processor} and 2D-torus \cite{kalray_mppa}.

From the routing point of view, a lot of algorithms have been proposed. They can be classified either in deterministic or adaptative category \cite{survey_wormhole}.
Due to our real-time concerns, we leave out adaptative routing algorithms and focus instead on deterministic routing algorithms. 
These ensure that the path of a packet in the network only ever depends on its source and destination. They are, however, unable to dynamically react to congestion.
The main concern of such algorithms is to prevent deadlocks (packets waiting for a resource forever) due to cyclic dependencies in the resources requested by flows.
They include dimension-ordered routing (the most common, can be X-Y or Y-X in 2D meshes), table-based routing, and turn-model routing \cite{survey_wormhole}.

Flow control mechanisms, on the other hand, determine how traffic is handled from router to router. 
Credit-based flow control is one of the most commonly used mechanisms. Each router holds as many credits as it has free space in its buffers, and a flit can move to the next router only if the router has a credit left for the corresponding buffer. 
This ensures a lossless transmission but can consequently induce backpressure when packets block each other, which makes timing analysis challenging.
To avoid backpressure phenomenon, one alternative from the flow control point of view is to use traffic shapers at the NoC interface level, as in \cite{kalray_mppa}. 
In this paper, we consider flow control mechanisms as one of our concerns is to bound backpressure impact on end-to-end delay.

The most relevant timing analyses of NoCs are mainly using two approaches: Scheduling Theory and Network Calculus, to which we can add ``hybrid'' methods such as Compositional Performance Analysis (CPA) and Recursive Calculus (RC). The main supported assumptions of each one of these analyses are summarized in Table \ref{tab:related_work_summary}, and we particularly consider: \begin{enumerate*}[label=(\roman*)] \item the use of \textit{wormhole routing} with \textit{multiple VCs}; 
\item the support of \textit{VCs Sharing} (\ie{} many traffic classes per VC) and \textit{priority Sharing} (\ie{} many traffic flows per priority level) in each router; 
\item the integration of the \textit{buffer size} and the flows \textit{serialization} impacts ;
\item the applicability of the model under CPQ and heterogeneous architectures assumptions. \end{enumerate*}
We did not include probabilistic approaches since they provide average delay estimations rather than worst-case guarantees suitable for real-time applications. 
Nonetheless it is worth to mention that such methods exist \cite{hu_app_buffer_alloc,kiasari2013_analytical_latency_model_noc}.

We now detail our review of the main timing analysis approaches.
%=============================================================================
Scheduling Theory (ST) has been used in \cite{burns_real_time_wormhole} to derive worst-case delay bounds in wormhole NoCs supporting multiple VCs and with no priority sharing. This method has been extended in \cite{burns_priority_share} to support the priority sharing. However, the latter approach may lead to overly pessimistic results for large NoCs with a high number of flows and a limited number of virtual channels. Moreover, the authors in \cite{xiong_2016_real_time_analysis_revisited} have proved later that the method in  \cite{burns_real_time_wormhole} could be optimistic in specific situations. They refined the response time analysis through the distinction between downstream and upstream indirect interferences, which leads to a deeper understanding of the problem. 
Although the authors exhibited a case of the ``multi-point progressive blocking'' (MPB) problem that caused the optimism in previous ST-based works, their initial approach still suffered from optimistic behaviour, that they later corrected in \cite{xiong_extending_rt_analysis_nocs}. 
However, they focus only on configurations with no priority sharing, which limits the applicability of such a proposal. 
Interesting enhancements of the work in \cite{burns_priority_share} have been detailed in \cite{liu_tighter_time_analysis}, where refined interference patterns between flows have been proposed through accounting for the physical contention domain impact, but considering only one-flit size buffers.
Finally, \cite{indrusiak2018_buffer_aware_mpb} attempted to refine the model of \cite{xiong_extending_rt_analysis_nocs}, noticing that the amount of flits causing MPB-related latency to the flow of interest (\emph{foi}) cannot exceed the total buffer size on the considered part of the \emph{foi} path to its destination. 
Nonetheless they provided no formal proof to their approach and instead relied on experimental results to support the validity of their model. 
Besides, these models do not consider non-CBR traffic.

%==============================================================================
Recently, the authors in \cite{Rambo:2015:WCT} have developed a model based on CPA, supporting priority sharing and VC sharing but ignoring the buffer backpressure. Afterwards, they have extended this work to support the backpressure in \cite{tobuschat_ernst_cpa_noc_backpressure}. However, the proposed analysis has considered only a single VC and buffer sizes that do not go below one packet. This analysis has also ignored the flows serialization phenomena.

%ADDED
Another recent work \cite{liu_buffer_aware} proposed a revision of Recursive Calculus \cite{ferrandiz_recursive_calculus}, correcting the optimism it induces when considering buffers that can contain more than one flit.
It also allows to model packet fragmentation (absent from most other approaches). Packet fragmentation is the way to transmit an amount of data exceeding the maximal packet size by splitting the data chunk into several packets.
However, their work does not account for traffic specificities such as packet interarrival time, nor for multiple VCs.

%==============================================================================
Finally, there are some recent works based on Network Calculus. In \cite{qian_analysis_worst_case_delays_wormhole}, the authors have solved the chain blocking problem due to the wormhole routing in a recursive way, through modeling the flow control system as a router component, whose behavior depends on the following router. This method infers complex fixed-point problems solving and has been validated only on relatively small NoCs with a simple flows configuration; thus limiting their approach applicability and scalability. Moreover, they have considered only a single-VC NoC routers.
Afterwards, the authors in \cite{jafari_ludb_vbr_flows_noc_vc} have provided tighter delay bounds, using improved arrival and service curves while taking buffer size and flows serialization into account. However, their approach seeks to provide a buffer size threshold to avoid the buffer backpressure. In addition, they do not consider wormhole routing as the switching technique; thus avoiding the complex chain blocking issue.
%ADDED
In \cite{boyer_computing_routes_kalray}, the authors computed end-to-end delay bounds on the Kalray MPPA2 Processor based on Network Calculus. This work is interesting from a practical perspective but it remains very specific to one architecture. The authors also assume traffic shapers are used to avoid backpressure and the buffer size is significantly bigger than all considered packet sizes.
The authors in \cite{buffer_aware} have started the exploration of the buffer size impact on the interference patterns. However, the considered wormhole routers do not support the VC concept and the proposed approach does not integrate the flows serialization phenomena.
Finally, our previous work \cite{giroudot_buffer_aware}, referred to as ``BATA'' approach from this point on, tried to fill the gaps of the previous approaches. 
We proposed a model handling VC sharing and priority sharing on NoCs, applicable to deterministically-routed configurations, and taking into account both limited buffer sizes and serialization phenomena. 
In this previous approach, we assumed that there cannot be more than one consecutive packet of the same flow in the network for flows indirectly impacting the flow of interest, \ie{} that CPQ does not occur. 
In particular, this does not alow to consider bursty traffic flows.
%If a packet of a non-bursty flow is delayed enough to impact the next injected packet of the same flow, such a scenario of consecutive-packet-queueing could also occur.

%This assumption is implicitely made in other works \cite{}, but for the flow under analysis rather than interfering flows. In our NC-based approach, we account for the potential non-schedulatbility of the \emph{foi} thanks to the burst propagation inherent to the underlying Network Calculus Theory.

%============our contributions===================================
As illustrated in Table \ref{tab:related_work_summary}, there is no existing timing analysis approach, which covers all the technical characteristics of wormhole NoC routers and supports the buffer size and flows serialization phenomena, along with being applicable whether or not CPQ occurs. 
%Hence, our main contribution in this paper is to cope with these different characteristics and assumptions to compute accurate end-to-end delay bounds in wormhole NoCs, using Network Calculus.
%% REFORMULATION
Hence, we propose an approach \begin{enumerate*}[label=(\roman*)] \item applicable to wormhole NoCs with multiple VCs, any buffer size, and heterogeneous characteristics; 
\item allowing to model priority-based traffic classes containing any number of flows; \item supporting the mapping of several priority classes to one VC; 
\item taking into account flow serialization; and \item covering CPQ scenarios.\end{enumerate*}
We base our model on Network Calculus theory.
%%ADDED
%{\color{blue}
%Moreover, we want our model to be as general as possible.
%As noticed by \cite{liu_buffer_aware}, most COTS platforms use Round-Robin-Arbitration (RRA) based NoCs instead of Fixed Priority (FP) based NoCs.
%While this concern is valid, we still chose to consider NoCs with virtual channels implementing priority classes given that \begin{enumerate*}[label=(\roman*)] \item traffic classes with priorities prove themselves useful when dealing with mixed-criticality traffic and \item our model can account for any multiplexing policy through the assumption of blind multiplexing.\end{enumerate*}
%}

